SceneTether: Activity-Gated Value Anchoring for Long-Horizon Autoregressive Image Animation

Long-horizon image animation must keep the scene fixed while natural material (e.g., water, smoke, or fire) continues to move. Autoregressive video generators read recent frames for temporal continuity, but this history also carries accumulated appearance errors, and sparsifying it disrupts motion. We introduce SceneTether, a training-free attention-read policy that keeps where attention reads recent memory but changes what appearance that memory returns. SceneTether keeps every key of the newest latent, blends its low-activity values toward co-located source-image values, and leaves high-activity values untouched so motion can evolve; an activity map estimated from the first generated latents and then frozen decides where to blend. It adds no denoising evaluations and leaves the cache-update rule unchanged. On a Causal Forcing++ generator, SceneTether raises source-support PSNR by 5.15 dB over its framewise Echo host across two seeds with 1.5x its late activity, and by 7.31 dB over spatial Echo-Forcing on a preselected four-minute subset. At equal recent-memory coverage, value anchoring alone adds 8.14 dB. A post-hoc pixel composite with the same map matches static fidelity but retains nearly twice the moving-region color drift, and viewers in a small blinded study preferred SceneTether for its natural scene and motion preservation. Project page: https://minar09.github.io/scenetether/

==> figures/method_diagrams_nov06/tether_patch.tex <==
% generated by tools/paper/build_method_diagrams_nov06.py; do not edit%
% window rows 13-16, cols 29-35 of the 30x52 token map%
\definecolor{tpr00}{RGB}{173,132,99}%
\definecolor{tps00}{RGB}{173,151,113}%
\definecolor{tpt00}{RGB}{173,148,111}%
\definecolor{tpr01}{RGB}{169,127,94}%
\definecolor{tps01}{RGB}{191,168,130}%
\definecolor{tpt01}{RGB}{191,168,130}%
\definecolor{tpr02}{RGB}{126,93,66}%
\definecolor{tps02}{RGB}{164,143,109}%
\definecolor{tpt02}{RGB}{164,143,109}%
\definecolor{tpr03}{RGB}{102,73,49}%
\definecolor{tps03}{RGB}{121,104,76}%
\definecolor{tpt03}{RGB}{111,88,62}%
\definecolor{tpr04}{RGB}{90,63,40}%
\definecolor{tps04}{RGB}{97,80,54}%
\definecolor{tpt04}{RGB}{95,76,51}%
\definecolor{tpr05}{RGB}{93,63,41}%
\definecolor{tps05}{RGB}{106,86,58}%
\definecolor{tpt05}{RGB}{106,86,58}%
\definecolor{tpr06}{RGB}{77,51,34}%
\definecolor{tps06}{RGB}{91,72,46}%
\definecolor{tpt06}{RGB}{88,69,44}%
\definecolor{tpr10}{RGB}{245,215,176}%
\definecolor{tps10}{RGB}{221,207,177}%
\definecolor{tpt10}{RGB}{233,211,177}%
\definecolor{tpr11}{RGB}{241,207,169}%
\definecolor{tps11}{RGB}{221,208,178}%
\definecolor{tpt11}{RGB}{231,207,173}%
\definecolor{tpr12}{RGB}{214,179,149}%
\definecolor{tps12}{RGB}{219,204,173}%
\definecolor{tpt12}{RGB}{216,191,161}%
\definecolor{tpr13}{RGB}{200,163,136}%
\definecolor{tps13}{RGB}{208,192,161}%
\definecolor{tpt13}{RGB}{204,178,149}%
\definecolor{tpr14}{RGB}{190,159,131}%
\definecolor{tps14}{RGB}{206,190,159}%
\definecolor{tpt14}{RGB}{192,162,133}%
\definecolor{tpr15}{RGB}{179,149,121}%
\definecolor{tps15}{RGB}{198,180,148}%
\definecolor{tpt15}{RGB}{190,167,137}%
\definecolor{tpr16}{RGB}{140,111,86}%
\definecolor{tps16}{RGB}{175,158,126}%
\definecolor{tpt16}{RGB}{174,156,125}%
\definecolor{tpr20}{RGB}{195,172,152}%
\definecolor{tps20}{RGB}{190,179,159}%
\definecolor{tpt20}{RGB}{195,172,152}%
\definecolor{tpr21}{RGB}{199,176,156}%
\definecolor{tps21}{RGB}{197,186,165}%
\definecolor{tpt21}{RGB}{198,181,160}%
\definecolor{tpr22}{RGB}{200,176,157}%
\definecolor{tps22}{RGB}{194,183,162}%
\definecolor{tpt22}{RGB}{200,176,157}%
\definecolor{tpr23}{RGB}{198,177,154}%
\definecolor{tps23}{RGB}{193,182,162}%
\definecolor{tpt23}{RGB}{196,180,158}%
\definecolor{tpr24}{RGB}{197,175,152}%
\definecolor{tps24}{RGB}{198,186,165}%
\definecolor{tpt24}{RGB}{197,180,158}%
\definecolor{tpr25}{RGB}{195,171,150}%
\definecolor{tps25}{RGB}{202,190,168}%
\definecolor{tpt25}{RGB}{199,180,159}%
\definecolor{tpr26}{RGB}{199,173,152}%
\definecolor{tps26}{RGB}{199,187,165}%
\definecolor{tpt26}{RGB}{199,180,159}%
\definecolor{tpr30}{RGB}{172,148,131}%
\definecolor{tps30}{RGB}{138,130,118}%
\definecolor{tpt30}{RGB}{172,148,131}%
\definecolor{tpr31}{RGB}{170,147,130}%
\definecolor{tps31}{RGB}{138,131,118}%
\definecolor{tpt31}{RGB}{170,147,130}%
\definecolor{tpr32}{RGB}{175,152,135}%
\definecolor{tps32}{RGB}{148,140,126}%
\definecolor{tpt32}{RGB}{175,152,135}%
\definecolor{tpr33}{RGB}{174,151,133}%
\definecolor{tps33}{RGB}{146,138,124}%
\definecolor{tpt33}{RGB}{174,151,133}%
\definecolor{tpr34}{RGB}{171,150,132}%
\definecolor{tps34}{RGB}{141,133,120}%
\definecolor{tpt34}{RGB}{171,150,132}%
\definecolor{tpr35}{RGB}{176,153,134}%
\definecolor{tps35}{RGB}{154,145,130}%
\definecolor{tpt35}{RGB}{165,149,132}%
\definecolor{tpr36}{RGB}{182,157,138}%
\definecolor{tps36}{RGB}{152,143,128}%
\definecolor{tpt36}{RGB}{182,157,138}%
\def\tpcells{0/0/0.82/0,0/1/1.00/0,0/2/1.00/0,0/3/0.49/0,0/4/0.77/0,0/5/1.00/0,0/6/0.85/0,1/0/0.50/0,1/1/0.50/0,1/2/0.50/0,1/3/0.50/0,1/4/0.08/0,1/5/0.59/0,1/6/0.97/0,2/0/0.00/1,2/1/0.50/0,2/2/0.00/1,2/3/0.50/0,2/4/0.50/0,2/5/0.50/0,2/6/0.50/0,3/0/0.00/1,3/1/0.00/1,3/2/0.00/1,3/3/0.00/1,3/4/0.00/1,3/5/0.50/0,3/6/0.00/1}%

